Image Difference Captioning with Pre-training and Contrastive Learning

The Image Difference Captioning (IDC) task aims to describe the visual differences between two similar images with natural language. The major challenges of this task lie in two aspects: 1) fine-grained visual differences that require learning stronger vision and language association and 2) high-cost of manual annotations that leads to limited supervised data. To address these challenges, we propose a new modeling framework following the pre-training-finetuning paradigm. Specifically, we design three self-supervised tasks and contrastive learning strategies to align visual differences and text descriptions at a fine-grained level. Moreover, we propose a data expansion strategy to utilize extra cross-task supervision information, such as data for fine-grained image classification, to alleviate the limitation of available supervised IDC data. Extensive experiments on two IDC benchmark datasets, CLEVR-Change and Birds-to-Words, demonstrate the effectiveness of the proposed modeling framework. The codes and models will be released at https://github.com/yaolinli/IDC.

==> history.tex <==
% \begin{small}
% \begin{equation}
%     \mathcal{L}_{\text{FDA}}=\\
%     \mathbb{E}_{V,T \in D}\left[
%         -\log \frac{\exp \left(d\left(V^{+}, T^{+}\right) / \tau_{2}\right)}
%         {\sum_{ \{-,+\}} \exp \left(d\left(V^{\prime}, T^{\prime}\right) / \tau_{2}\right)}
%     \right]
% \end{equation}
% \end{small}

\begin{small}
\begin{equation}
    -\log 
        \frac{ \exp \left(d(\hat{v}_{m}, v_{m}^{+}) / \tau_{1} \right)}
        {\sum_{v^{\prime} \in \hat{V}} \exp \left(d(\hat{v}_{m}, v^{\prime}) / \tau_{1} \right)}
\end{equation}
\end{small}

% SOTA on CLEVR
\begin{table}[htb] 
\begin{center}
% \small
\begin{tabular}{l|ccc >{\columncolor[gray]{0.9}} c}
\toprule
\multirow{2}{2cm}{\textbf{Model}}  & \multicolumn{4}{c}{\textbf{CLEVR-Change}}   \\
 & B4        & M        & R       & \textbf{C}     \\ \midrule
Capt-Dual-Att~\shortcite{park2019robust} &43.5 &32.7 &- &108.5 \\
DUDA~\shortcite{park2019robust} & 47.3 & 33.9 & - & 112.0 \\
VAM~\shortcite{shi2020finding} & 50.3 & 37.0 & 69.7 & 114.9 \\
VAM+~\shortcite{shi2020finding} & \textbf{51.3} & \textbf{37.8} & 70.4 & 115.8 \\
IFDC~\shortcite{tmm} & 49.2 & 32.5 & 69.1 & 118.7 \\
DUDA+Aux~\shortcite{2021Auxiliary} & 51.2 &37.7 &70.5 & 115.4 
\\\midrule
Ours &51.2 &36.2 &\textbf{71.7} &\textbf{130.9}   \\
\bottomrule
\end{tabular}
\end{center}
\caption{Comparison of our model with state-of-the-art models on CLEVR-Change dataset. The main metric of this dataset is \textbf{CIDEr}. B4 is short for BLEU-4, M for METEOR, R for ROUGE-L, C for CIDEr. 
}
\label{tab:SOTA_CLEVR}
\end{table}

% break down different types in CLEVR-Change dataset
\begin{table}[htb]
\begin{center}
% \small
\begin{tabular}{l|cccccc}
\toprule
\multirow{2}{1cm}{\textbf{Model}}  & \multicolumn{6}{c}{\textbf{CIDEr}}   \\
 & C  & T  & M  & A & D & DI    \\ \midrule
DUDA~ & 120.4 & 86.7 & 56.4 & 108.2 &103.4 &110.8 \\
VAM+~ & 122.1 & 98.7 & 82.0 & 126.3 &115.8 &122.6 \\
IFDC~ & 133.2 & 99.1 & 82.1 & 128.2 &118.5 &114.2 \\
\midrule
Ours  & \textbf{137.0} & \textbf{105.7} & \textbf{84.9} & \textbf{136.1} &\textbf{120.3} &\textbf{145.0}  \\
\bottomrule
\end{tabular}
\end{center}
\caption{Breakdown CIDEr performance of CLEVR-Change Dataset on different type changes: C (Color), T (Texture), M (Move), A (Add), D (Drop) and DI (Distractor).  
}
\label{tab:CLEVR_type}
\end{table}

\begin{table}[htb]
\begin{center}
% \small
\begin{tabular}{l|ccc >{\columncolor[gray]{0.9}} c}
\toprule
\multirow{2}{2cm}{\textbf{Model}} &  \multicolumn{4}{c}{\textbf{Birds-to-Words}} \\
&B4        & M       & C(D)    & \textbf{R} \\ \midrule
Neural Naturalist~\shortcite{forbes2019neural}  & 22.0 & - & 25.0  & 43.0          \\
Relational Speaker~\shortcite{tan2019expressing} & 21.5 & 22.4 & 5.8 & 43.4  \\
DUDA~\shortcite{park2019robust}  & 23.9 & 21.9 & 4.6 & 44.3   \\ 
L2C~\shortcite{yan2021l2c} & 31.3 & - & 15.1 & 45.3 \\
L2C(+CUB)~\shortcite{yan2021l2c} & \textbf{31.8} & - & 16.3 & 45.6   \\ \midrule
Ours &28.0 &23.1 &18.6  &48.4   \\
Ours(+Extra Data) &31.0 &\textbf{23.4} &\textbf{25.3}  &\textbf{49.1}  \\
\bottomrule
\end{tabular}
\end{center}
\caption{Comparison of our model with other state-of-the-art models on Birds-to-Words dataset. The main metric of Birds-to-Words dataset is \textbf{ROUGE-L}. B4 is short for BLEU-4, M for METEOR, R for ROUGE-L, C(D) for CIDEr-D. 
}
\label{tab:SOTA_Bird}
\end{table}

% Ablation Study
\begin{table*}[htb]
\begin{center}
% \small
\begin{tabular}{c|l|c|ccc >{\columncolor[gray]{0.9}} c}
\toprule

\textbf{Line}   & \textbf{Pre-training Tasks}   & \textbf{Diff Enc}   & B4        & M        & R  & \textbf{C}    \\ 
 \midrule
1    & - & \checkmark &32.7 &27.7 &57.2 &91.3   \\
% 6  & \XSolidBrush  &  None    &36.8 &30.2 &61.5 &96.4   \\
2    & \text{MLM } & \checkmark &36.7  &28.2   &60.9   &96.9   \\
3    & \text{MLM +  \text{MVCL} } & \checkmark &50.3 &37.6 &70.6 &121.5\\
4    & \text{MLM  +  \text{MVCL} + \text{FDA}} & \checkmark  &51.2 &36.2 &71.7 &130.9   \\
\midrule
5    & \text{MLM + MVFR + ITM} & \checkmark  &52.3 &35.1 &71.4 &126.3   \\
\midrule
6    & \text{MLM +  \text{MVCL} + \text{FDA}} & \XSolidBrush  &49.2 &35.8 &68.8 & 109.3   \\
%5  & \XSolidBrush  & \text{MLM + MVFR + ITM}  &47.9 &36.6 &69.2 &123.2  \\

\bottomrule
\end{tabular}
\end{center}
\caption{Ablation study results on CLEVR-Change dataset. \textbf{Diff Enc} is short for image difference encoder module in our model. 
}
\label{tab:Ablation}
\end{table*}



% data extension on Bird dataset
\begin{table*}[t]
\begin{center}
\small
\begin{tabular}{l|ccc|cccc >{\columncolor[gray]{0.9}}c}
\toprule
\textbf{Model} 
&B2W  &CUB  &NAB 
 & B4  & M   & C(D) &BS & \textbf{R}  \\ \midrule
\multirow{2}{1cm}{L2C} & \checkmark  & & & 31.3 & - & 15.1 &-  & 45.3 \\
 & \checkmark  &\checkmark   &           & 31.8 & - & 16.3 &-  & 45.6 \\

\midrule
\multirow{4}{1cm}{Ours}
% only bird
& \checkmark  &            &           &28.0 &23.1 &18.6  &27.3  &48.4 \\
% bird+CUB
& \checkmark  &\checkmark  &           &29.3 &23.1 &23.8 &32.1   &48.5 \\
% bird+NAbird
& \checkmark  &            &\checkmark &27.5 &23.3 &21.9 &30.2   &48.5 \\
% bird+CUB+NABird
& \checkmark  &\checkmark  &\checkmark &31.0 &23.4 &25.3 &32.7   &49.1 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Model performance on Birds-to-Words(B2W for short) dataset using two  cross-task dataset including CUB and NABirds(NAB for short). The main metric is \textbf{ROUGE-L(R)}. BS is short for BERTScore. 
}
\label{tab:in_domain}
\end{table*}

% \begin{table}[ht]
% \begin{center}
% \small
% \begin{tabular}{l|ccc|c >{\columncolor[gray]{0.9}}c}
% \toprule
% \textbf{Model} 
% &B2W  &CUB  &NAB 
%  &BS & \textbf{R}  \\ \midrule
% \multirow{2}{1cm}{L2C} & \checkmark  & & &-  & 45.3 \\
%  & \checkmark  &\checkmark   &            &-  & 45.6 \\

% \midrule
% \multirow{4}{1cm}{Ours}
% % only bird
% & \checkmark  &            &            &27.3  &48.4 \\
% % bird+CUB
% & \checkmark  &\checkmark  &            &32.1   &48.5 \\
% % bird+NAbird
% & \checkmark  &            &\checkmark  &30.2   &48.5 \\
% % bird+CUB+NABird
% & \checkmark  &\checkmark  &\checkmark  &32.7   &49.1 \\
% \bottomrule
% \end{tabular}
% \end{center}
% \caption{Model performance on Birds-to-Words(B2W for short) dataset using two  cross-task dataset including CUB and NABirds(NAB for short). The main metric is \textbf{ROUGE-L(R)}. BS is short for BERTScore. 
% }
% \label{tab:in_domain}
% \end{table}


% related works
\cite{jhamtani2018learning} collect  difference descriptions of street-view images extracted from video-surveillance footage. \cite{park2019robust} automatically constructs a scene change captioning dataset with distractors(viewpoint or illumination change). \cite{tan2019expressing} annotates image pairs from editing request websites with editing instructions. \cite{forbes2019neural} defines appearance differences between bird species in the wild with paragraph-length descriptions. 

For example, \cite{park2019robust} design a dual attention for the spacial semantic interaction between two images. \cite{tan2019expressing} explore the efficacy of sequential multi-head attention, static and dynamic relational attention. \cite{shi2020finding} propose a Reinforcement Attention Fine-tuning (RAF) strategy to enhance the designed attention. Other works focus on improving the visual representations. For example, \cite{yan2021l2c} reason and compare the semantic structures of two images, while \cite{tmm} consider the instance-level image features. 


\begin{small}
\begin{equation}
    -\log 
        \frac{ \exp \left(d(\hat{v}_{m}, v_{m}^{+}) / \tau_{1} \right)}
        {
            \sum_{v^{\prime} \in \{v_{m}^{+},\  \mathcal{N} \} } \exp \left(d(\hat{v}_{m}, v^{\prime}) / \tau_{1} \right)}
\end{equation}
\end{small}
where $d(.)$ is the inner product, $\tau_{1}$ is the temperature hyper-parameter, $\hat{v}_{m}$ denotes the output of $v_{m}$ from cross-modal transformer, $v_{m}^{+}$ denotes the original input image feature of $v_{m}$,  and $\mathcal{N}$=$\{\hat{v}_{\backslash m}\}$ is the set of output unmasked features  in the batch. The contrastive loss pushes the model to identify the positive sample $v_{m}^{+}$ of $\hat{v}_{m}$ from negative samples $\{\hat{v}_{\backslash m}\}$, which enforces the reconstructed image representations $\hat{v}_{m}$ to be more discriminative. 
